Maximum Likelihood Estimation is All You Need for Well-Specified Covariate Shift

A key challenge of modern machine learning systems is to achieve Out-of-Distribution (OOD) generalization -- generalizing to target data whose distribution differs from that of source data. Despite its significant importance, the fundamental question of ``what are the most effective algorithms for OOD generalization'' remains open even under the standard setting of covariate shift. This paper addresses this fundamental question by proving that, surprisingly, classical Maximum Likelihood Estimation (MLE) purely using source data (without any modification) achieves the minimax optimality for covariate shift under the well-specified setting. That is, no algorithm performs better than MLE in this setting (up to a constant factor), justifying MLE is all you need. Our result holds for a very rich class of parametric models, and does not require any boundedness condition on the density ratio. We illustrate the wide applicability of our framework by instantiating it to three concrete examples -- linear regression, logistic regression, and phase retrieval. This paper further complement the study by proving that, under the misspecified setting, MLE is no longer the optimal choice, whereas Maximum Weighted Likelihood Estimator (MWLE) emerges as minimax optimal in certain scenarios.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pf_mis_expectation_upper.tex <==
\subsection{Expectation upper bound}\label{mis:expectation_upper}
If we are given prior knowledge that $\beta^{\star}(M)\in\bbB_{\beta_0}(B)$ for some $\beta_0\in\bbR^{d}$ and $B>0$, then we consider the following constrained MWLE:
\begin{align*}
 \tilde{\beta}_{\MWLE}:=\argmin_{\beta\in\bbB_{\beta_0}(2B)}\frac1n \sum^n_{i=1}w(x_i)\ell(x_i,y_i,\beta).   
\end{align*}

% \begin{corollary}\label{cor:mis_upper}
% Suppose $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \min \left\{ \frac{1}{W\tilde{B}(M)\|H^{-1}_w(M)\|_{2}\sqrt{\Tr(G_w(M)H^{-2}_w(M))}}, \frac{B}{\sqrt{\Tr(G_w(M)H^{-2}_w(M))}} \right\}$. Under Assumptions \ref{assm1_mis}, \ref{assm2_mis}, \ref{assm3_mis} and \ref{assm6}, we have
% \begin{align*}
% \bbE_{(x_i,y_i)\sim\bbP_S(X,Y)}\left[R_{M}(\tilde{\beta}_{\MWLE})\right] &\leq \frac{c\Tr\left(G_w(M)H^{-1}_w(M)\right)}{n} \\
% &+ \cO \left(W\tilde{B}(M) \Tr(G_w(M)H^{-2}_w(M))^{1.5} \left(\frac{\log (n^{10}d)}{n}\right)^{1.5}  + \frac{W\tilde{B}(M)B^{3}\|H_w(M)\|_2 }{n^{10}} \right)
% \end{align*}
% where $\tilde{B}(M) := \max \{B_1(M), B_2(M), B_3\},$
% $c$ is an absolute constant and $\cO(\cdot)$ only omits absolute constants.
% \end{corollary}

\begin{corollary}\label{cor:mis_upper}
Suppose Assumptions \ref{assm1_mis}, \ref{assm2_mis}, \ref{assm3_mis} and \ref{assm6} hold. We have
\begin{align*}
\bbE_{(x_i,y_i)\sim\bbP_S(X,Y)}\left[R_{M}(\tilde{\beta}_{\MWLE})\right] &\lesssim\frac{\Tr\left(G_w(M)H^{-1}_w(M)\right)}{n}    
\end{align*}
when 
\begin{align*}
n\gtrsim \max\bigg\{
&W^2\tilde{B}(M)^2\|H^{-1}_w(M)\|^2_{2}\Tr(G_w(M)H^{-2}_w(M))\log d W\tilde{B}(M)\|H^{-1}_w(M)\|_{2}\Tr(G_w(M)H^{-2}_w(M)),\\
& \frac{W^2\tilde{B}(M)^2 \Tr(G_w(M)H^{-2}_w(M))^{3}}{\Tr\left(G_w(M)H^{-1}_w(M)\right)^2}\left(\log d W\tilde{B}(M) \Tr(G_w(M)H^{-2}_w(M))\right)^3
\bigg\}.
\end{align*}
Here $\tilde{B}(M) := \max \{B_1(M), B_2(M), B_3\}$.
\end{corollary}


\begin{proof}[Proof of Corollary \ref{cor:mis_upper}]
In the proof of Theorem \ref{thm:mis_upper}, we already have with probability at least $1-2\delta -2/n^{10}$,
\begin{align*} 
R_{M}(\beta_{\MWLE})  &\lesssim \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*}
Also notice that, under this event, since $\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}} \leq B$, by Lemma \ref{claim1_mis}, $\beta_{\MWLE}\in\bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}}) \subset \bbB_{\beta_{0}}(2B)$. Thus $\beta'_{\MWLE}=\beta_{\MWLE}$. Therefore we have with probability at least $1-2\delta -2/n^{10}$, 
\begin{align}\label{ineq:pf:upper1_mis} 
&R_{M}(\beta'_{\MWLE})  \notag\\
&\lesssim \underbrace{ \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})}_{=:f(\delta)}.
\end{align}
Taking the expectation, we have
\begin{align} \label{ineq:pf:upper2_mis}
& \bbE_{(x_i,y_i)\sim \bbP_{S}(X,Y)}\left[R_{M}(\beta_{\MWLE})\right] \notag \\
& = \int_{0}^{+\infty} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t \notag \\
&= \underbrace{\int_{0}^{f(1)} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t }_{=
:K_1}+ \underbrace{\int_{f(1)}^{f(\frac{1}{n^{10}})} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t }_{=:K_2}+ \underbrace{\int_{f(\frac{1}{n^{10}})}^{+\infty} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t }_{=:K_3}.
\end{align}
We will relatively bound these three terms $K_1, K_2, K_3$.
Note that
\begin{align} \label{ineq:pf:upper3_mis}
K_{1} &=  \int_{0}^{f(1)} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t \notag \\
& \leq \int_{0}^{f(1)} 1 \mathrm{d}t \notag \\
&= f(1) \notag \\
&= \cO \left(  W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} \right),
\end{align}
where the last equality holds because of the definition of $f(\delta)$  (see \eqref{ineq:pf:upper1_mis}).

\begin{align} \label{ineq:pf:upper4_mis}
K_2 &= \int_{f(1)}^{f(\frac{1}{n^{10}})} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t \notag \\
&\stackrel{\text{let } t=f(\delta)}{=} -\int_{\frac{1}{n^{10}}}^{1} \bbP(R_{M}(\beta_{\MWLE}) \geq f(\delta)) f'(\delta) \mathrm{d}\delta \notag \\
& \stackrel{\text{by (\ref{ineq:pf:upper1_mis}})}{\leq} -\int_{\frac{1}{n^{10}}}^{1} (2\delta + \frac{2}{n^{10}}) f'(\delta) \mathrm{d}\delta \notag \\
& = - 2\int_{\frac{1}{n^{10}}}^{1} \delta f'(\delta) \mathrm{d}\delta - \frac{2}{n^{10}} \int_{\frac{1}{n^{10}}}^{1} f'(\delta) \mathrm{d}\delta \notag \\
&= - 2\int_{\frac{1}{n^{10}}}^{1} \delta \frac{c \Tr(G_w H_w^{-1})}{n} \delta (-\frac{1}{\delta^{2}}) \mathrm{d}\delta -\frac{1}{n^{2}}  \|H_w^{-1}\|_2W^2 \tilde{B}^{2} \int_{\frac{1}{n^{10}}}^{1} \cO \left(\delta^{2}(-\frac{1}{\delta^{2}}) \log \frac{1}{\delta}\right) \mathrm{d}\delta - \frac{2}{n^{10}} (f(1)-f(\frac{1}{n^{10}})) \notag \\
&\leq  \frac{2c \Tr(G_w H_w^{-1})}{n} + \frac{1}{n^{2}} \|H_w^{-1}\|_2W^2 \tilde{B}^{2} \int_{0}^{1} \cO(\log \frac{1}{\delta})\mathrm{d}\delta + \frac{2}{n^{10}} f(\frac{1}{n^{10}}) \notag \\
& = \frac{2c \Tr(G_w H_w^{-1})}{n} + \cO(\frac{1}{n^{2}} \|H_w^{-1}\|_2W^2 \tilde{B}^{2})\notag\\
&\quad + \frac{1}{n^{10}}\cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5}  + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log n}{n})^{2})\notag \\
& \leq \frac{2c \Tr(G_w H_w^{-1})}{n} + \cO(\frac{1}{n^{2}} \|H_w^{-1}\|_2W^2 \tilde{B}^{2}),
\end{align}
where the last inequality follows from $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{W\tilde{B}(\beta^{\star})\| H^{-1}_w(\beta^{\star})\|_{2}\sqrt{\Tr(G_w(\beta^{\star})H^{-2}_w(\beta^{\star}))}}$


Note that $\beta^{\star}, \beta_{\MWLE} \in \bbB_{\beta_{0}}(2B)$, we have a trivial bound
\begin{align*}
R_{M}(\beta_{\MWLE}) \leq \frac{1}{2}(\beta_{\MWLE}-\beta^{\star})^{T}H_w(\beta_{\MWLE}-\beta^{\star}) +\frac{WB_{3}}{6}\|\beta_{\MWLE}-\beta^{\star}\|_{2}^{3} \lesssim \|H_w\|_{2}W\tilde{B}B^{3}.
\end{align*}
Thus 
\begin{align} \label{ineq:pf:upper5_mis}
K_3 &= \int_{f(\frac{1}{n^{10}})}^{+\infty} \bbP(R_{M}(\beta_{\MWLE}) \geq t) \mathrm{d}t \notag \\
& = \bbE_{(x_i,y_i) \sim \bbP_{S}(X,Y)}\left[(R_{M}(\beta_{\MWLE})- f(\frac{1}{n^{10}})) \bbI_{(R_{M}(\beta_{\MWLE})- f(\frac{1}{n^{10}})\geq 0)}\right] \notag \\
& \leq \|H_w\|_{2}W\tilde{B}B^{3} \bbP(R_{M}(\beta_{\MWLE}) \geq f(\frac{1}{n^{10}})) \notag \\
& \lesssim \frac{1}{n^{10}}\|H_w\|_{2}W\tilde{B}B^{3}
\end{align}
Combine  (\ref{ineq:pf:upper2_mis}), (\ref{ineq:pf:upper3_mis}), (\ref{ineq:pf:upper4_mis}) and (\ref{ineq:pf:upper5_mis}), notice that $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{W\tilde{B}(\beta^{\star})\| H^{-1}_w(\beta^{\star})\|_{2}\sqrt{\Tr(G_w(\beta^{\star})H^{-2}_w(\beta^{\star}))}}$, we have 
\begin{align*}
&\bbE_{(x_i,y_i) \sim \bbP_{S}(X,Y)}\left[R_{M}(\beta_{\MWLE})\right] \leq \frac{c \Tr(G_w H_w^{-1})}{n} + \cO \left(W\tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5}+ \frac{\|H_w\|_{2}W\tilde{B}B^{3}}{n^{10}}\right),
\end{align*}
where $c$ is an absolute constant and $\cO(\cdot)$ only omits absolute constants.


\end{proof}


==> pf_v1_linear_regression.tex <==
\subsection{Proofs for Theorem \ref{thm:linear}}\label{pf:thm_linear}
\begin{proof}[Proofs for Theorem \ref{thm:linear}]
In this section, we aim to prove the upper bound of MLE for linear regression model. We can not directly apply Theorem \ref{thm:well_upper} since Assumption \ref{assm1} is not satisfied. Notice that, in the proof of Theorem \ref{thm:well_upper}, the only use of Assumption \ref{assm1} is to derive concentrations (\ref{ineq:pf:concentration1}) and (\ref{ineq:pf:concentration2}) (by Lemma \ref{lem:bernstein} with bounded random vectors). Therefore we can apply a modified version of Lemma \ref{lem:bernstein} for norm-sub-Gaussian random vectors and gain the corresponding concentration inequalities for proving Theorem \ref{thm:linear} in the same way of proving Theorem \ref{thm:well_upper}.

\begin{lemma}
\label{lem:bernstein2}
Let $u_{1},\cdots,u_{n}$ be i.i.d. mean-zero random vectors such that 
\begin{align*}
    \bbE[\|u_{i}\|^{2}_{2}] \leq v \quad \text{and } \quad \bbP(\|u_{i}\|_{2} \geq t) \leq 2e^{-\frac{t^{2}}{2B^{2}}}
\end{align*}
for all $i=1, \cdots, n$, almost surely. Then for any $\delta \in (0,e^{-1})$, with probability at least $1-\delta-\frac{2}{n^{10}}$,
\begin{align*}
     \|\frac{1}{n}\sum_{i=1}^{n}u_{i}\|_{2} \leq  \sqrt{\frac{v}{n}} +\sqrt{\frac{8v\log \frac{1}{\delta}}{n}}+CB\frac{\sqrt{\log n}\log \frac{1}{\delta}}{n}
\end{align*}
for some absolute constant $C$.
\end{lemma}
With this lemma, we can now derive the corresponding concentrations. For our linear regression model, 
\begin{align*}
\ell(x,y,\beta) = \frac{1}{2}\log (2 \pi) + \frac{1}{2} (y-x^{T}\beta)^{2}.    
\end{align*}
We then have
\begin{align*}
&\nabla\ell(x,y,\beta)
=-x(y-x^{T}\beta),\\
&\nabla^2\ell(x,y,\beta)
=xx^T,\\
&\nabla^3\ell(x,y,\beta)
=0, \\
& \cI_(S)=\bbE_{x\sim\bbP_S(X)}[xx^T] =\Sigma_S, \\
& \cI_(T)=\bbE_{x\sim\bbP_T(X)}[xx^T] =\Sigma_T.
\end{align*}
It's obvious that linear regression satisfies Assumption \ref{assm1} and \ref{assm2} with $B_2=D^{2}$, $B_3=0$. For the gradient bound, for any matrix $A\in \bbR^{d \times d}$, if we choose $u_{i}:=A(\nabla \ell (x_{i},y_{i}, \beta^{\star}) - \bbE_{\bbP_{S}}[\nabla \ell (x,y, \beta^{\star})])$, then 
\begin{align*}
u_{i}&=A(\nabla \ell (x_{i},y_{i}, \beta^{\star}) - \bbE_{\bbP_{S}}[\nabla \ell (x,y, \beta^{\star})]) \\
&= A (-x_i(y_i-x_i^{T}\beta^{\star})) \\
&\stackrel{y_i = x_i^{T}\beta^{\star} + \epsilon_i}{=} -Ax_i \epsilon_i.
\end{align*}
Notice that $
\|-Ax_i \epsilon_i\| \leq \|A\| \|x_{i}\| \|\epsilon_i\| \leq D \|A\|  \|\epsilon_i\|$,
and $\epsilon_i \sim \mathcal{N}(0,1)$, which means $-Ax_i \epsilon_i$  satisfies the conditions in Lemma \ref{lem:bernstein2} with $B=D\|A\|$, $v=\Tr (A^{T}A\cI_{S})$. Let $g:= \nabla \ell_{n}(\beta^{\star}) - \nabla \ell(\beta^{\star})$, then we have with probability at least $1-\delta- \frac{2}{n^{10}}$, 
\begin{align*}
    \|Ag\|_{2} \leq \sqrt{\frac{\Tr(A^{T}A\cI_{S})}{n}}+  \sqrt{\frac{8\Tr(A^{T}A\cI_{S}) \log \frac{1}{\delta}}{n}}+ CD\|A\|\frac{\sqrt{\log n}\log \frac{1}{\delta}}{n},
\end{align*}
Choose $A= \cI_{S}^{-1}$ and $\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}$ relatively, we have
\begin{align} \label{ineq:pf:concentration1_linear}
    \|\cI_{S}^{-1}g\|_{2} \lesssim \sqrt{\frac{\Tr(\cI_{S}^{-1})}{n}}+  \sqrt{\frac{\Tr(\cI_{S}^{-1}) \log \frac{1}{\delta}}{n}}+ CD\|\cI_{S}^{-1}\|\frac{\sqrt{\log n}\log \frac{1}{\delta}}{n}
\end{align}
and 
\begin{align} \label{ineq:pf:concentration2_linear}
    \|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}g\|_{2} \lesssim \sqrt{\frac{\Tr(\cI_{S}^{-1}\cI_{T})}{n}}+  \sqrt{\frac{\Tr(\cI_{S}^{-1}\cI_{T}) \log \frac{1}{\delta}}{n}}+ CD\|\cI_{T}^{-\frac{1}{2}}\cI_{S}^{-1}\|\frac{\sqrt{\log n}\log \frac{1}{\delta}}{n}
\end{align}
with probability at least $1-\delta-\frac{2}{n^{10}}$ relatively. Notice that (\ref{ineq:pf:concentration1_linear})and (\ref{ineq:pf:concentration2_linear}) can be viewed as setting $B_1=D\sqrt{\log n}$ in \eqref{ineq:pf:concentration1} and \eqref{ineq:pf:concentration2}. Therefore we can prove Theorem \ref{thm:linear} by the same way of proving Theorem \ref{thm:well_upper}, with $B_1=D\sqrt{\log n}$, $B_2=D^{2}$, $B_3=0$ (let $\tilde{B}=D^{2}\sqrt{\log n}$). The verification of linear regression model satisfies Assumption \ref{assm3} is almost the same as in the previous section.

Finally we state the proof of Lemma \ref{lem:bernstein2}.
\begin{proof}[Proof of Lemma \ref{lem:bernstein2}]
By the sub-Gaussian assumption of $\|u_i\|$, we have 
\begin{align*}
\bbP(\exists i \in [n], \, s.t. \, \|u_i\| \geq \sqrt{22B^{2}\log n})     &\leq \sum_{i=1}^{n} \bbP( \|u_i\| \geq \sqrt{22B^{2}\log n}) \\
&\leq n \times 2 e^{-\frac{22B^{2}\log n}{2B^{2}}} \\
& = \frac{2}{n^{10}}.
\end{align*}
Let $\tilde{u}_i := u_i \bbI_{\{ \|u_i\| < \sqrt{22B^{2}\log n}\}} $, then
\begin{align*}
\|\bbE [\tilde{u}_i]\| &= \|\bbE[u_i] - \bbE [u_i\bbI_{\{ \|u_i\| \geq \sqrt{22B^{2}\log n}\}}] \| \\ 
&\stackrel{\bbE[u_i]=0}{=} \|\bbE [u_i\bbI_{\{ \|u_i\| \geq \sqrt{22B^{2}\log n}\}}] \| \\ 
& \leq \bbE [\|u_i\|\bbI_{\{ \|u_i\| \geq \sqrt{22B^{2}\log n}\}}]  \\
&= \int_{\sqrt{22B^{2}\log n}}^{\infty} \bbP(\|u_i\|\geq t) \mathrm{d} t  + \sqrt{22B^{2}\log n} \bbP(\|u_i\| \geq \sqrt{22B^{2}\log n}) \\
& \leq \int_{\sqrt{22B^{2}\log n}}^{\infty} 2e^{-\frac{t^{2}}{2B^{2}}} \mathrm{d} t  + \frac{2}{n^{11}}\sqrt{22B^{2}\log n}  \\
& \stackrel{\text{let } t=Bs}{=} \int_{\sqrt{22 \log n}}^{\infty} 2Be^{-\frac{s^{2}}{2}} \mathrm{d} s  + \frac{2}{n^{11}}\sqrt{22B^{2}\log n}  \\
&= cB \bbP(\cN (0,1) \geq \sqrt{22 \log n})  + \frac{2}{n^{11}}\sqrt{22B^{2}\log n}  \\
& \stackrel{\text{by Gaussian tail bound}}{\leq} cB e^{-\frac{22\log n }{2}}+ \frac{2}{n^{11}}\sqrt{22B^{2}\log n}  \\
& \leq CB \frac{\sqrt{\log n}}{n^{11}}.
\end{align*}
Thus 
\begin{align*}
\|\tilde{u}_i - \bbE \tilde{u}_i\| &\leq \|\tilde{u}_i\|+ \|\bbE \tilde{u}_i\| \\
& \leq \sqrt{22B^{2}\log n} +  CB \frac{\sqrt{\log n}}{n^{11}} \\
& \leq CB \sqrt{\log n}.
\end{align*}
Moreover, 
\begin{align*}
\bbE[\|\tilde{u}_i - \bbE \tilde{u}_i\|^{2}] = \bbE[\|\tilde{u}_i\|^{2}] -\| \bbE \tilde{u}_i\|^{2} \leq \bbE[\|\tilde{u}_i\|^{2}] \leq \bbE[\|u_i\|^{2}].
\end{align*}
Therefore we can apply Lemma \ref{lem:bernstein} to $\tilde{u}_i - \bbE \tilde{u}_i$ as the random vector sequence, which gives
\begin{align*}
\bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i - \bbE \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n}) \leq \delta,
\end{align*}
which implies 
\begin{align*}
\bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n} + CB \frac{\sqrt{\log n}}{n^{11}}) \leq \delta,
\end{align*}
since $\|\bbE \tilde{u}_i\| \leq CB \frac{\sqrt{\log n}}{n^{11}}$. Thus we have
\begin{align*}
& \bbP (\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n} + CB \frac{\sqrt{\log n}}{n^{11}})   \\
&= \bbP (\{\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n} + CB \frac{\sqrt{\log n}}{n^{11}}\} \cap \{\exists i \in [n], \, s.t. \, \|u_i\| \geq \sqrt{22B^{2}\log n}\}) \\
&+\bbP (\{\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n} + CB \frac{\sqrt{\log n}}{n^{11}}\} \cap \{\forall i \in [n], \,  \, \|u_i\| < \sqrt{22B^{2}\log n}\})  \\
& \leq \bbP(\exists i \in [n], \, s.t. \, \|u_i\| \geq \sqrt{22B^{2}\log n}) + \bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4CB\sqrt{\log n} \log \frac{1}{\delta}}{3n} + CB \frac{\sqrt{\log n}}{n^{11}})   \\
& \leq \frac{2}{n^{10}} + \delta.
\end{align*}
Notice that for $\delta \in (0,e^{-1})$, $\log \frac{1}{\delta} \geq 1$, we immediately get what we want.
\end{proof}
\end{proof}


==> pf_v1_mis_upper_bound.tex <==
\subsection{Proofs for Theorem \ref{thm:mis_upper}}
The proofs for Theorem \ref{thm:mis_upper} and Corollary \ref{cor:mis_upper} are similar to proofs for Theorem \ref{thm:well_upper} and \ref{cor:well_upper}. For notation simplicity, through out the proofs for Theorem \ref{thm:mis_upper}, let $\beta^{\star}:=\beta^{\star}(M)$, $H_w:= H_w(M)$, $  G_w:= G_w(M)$, $B_1:=B_1(M)$, $B_2:=B_2(M)$, $\tilde{B}:=\tilde{B}(M)$. With little abuse of notation, through out the this section, let 
\begin{align*}
\ell_n(\beta):=\frac1n \sum^n_{i=1}w(x_i)\ell(x_i,y_i,\beta).
\end{align*}
Then 
\begin{align*}
\beta_{\MWLE}=\argmin_{\beta\in\bbR^d}\ell_n(\beta).
\end{align*}
Note that  
\begin{align*}
\bbE_{(x_i,y_i) \sim \bbP_S(X,Y)}\ell_n(\beta)= \bbE_{(x,y) \sim \bbP_S(X,Y)}[w(x)\ell(x,y,\beta)]=  \bbE_{(x,y) \sim \bbP_T(X,Y)}[\ell(x,y,\beta)],
\end{align*}
by definition, 
\begin{align*}
\beta^{\star}=\argmin_{\beta\in\bbR^d}\bbE_{(x_i,y_i) \sim \bbP_S(X,Y)}[\ell_n(\beta)].
\end{align*}
We first state two main lemmas. Informally speaking, Lemma \ref{claim1_mis} shows that $\beta_{\MWLE}$ falls in a ball around $\beta^{\star}$ with radius $\sqrt{\frac{\log n}{n}}$. With Lemma \ref{claim1_mis}, Lemma \ref{claim2_mis} gives a high probability bound for $\beta_{\MWLE}- \beta^{\star}$. 

\begin{lemma}\label{claim1_mis}
Suppose $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{W\tilde{B}(\beta^{\star})\| H^{-1}_w(\beta^{\star})\|_{2}\sqrt{\Tr(G_w(\beta^{\star})H^{-2}_w(\beta^{\star}))}}$. Under Assumptions \ref{assm1_mis}, \ref{assm2_mis}, \ref{assm3_mis} and \ref{assm6}, we have with probability at least $1-2/n^{10}$,  $\beta_{\MWLE}\in\bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w(\beta^{\star})H^{-2}_w(\beta^{\star}))\log (n^{10}d)}{n}})$, where $\tilde{B}:= \max \{B_1,B_2,B_3\}$.
\end{lemma}


\begin{lemma}\label{claim2_mis}
Under same conditions as in Lemma \ref{claim1_mis}. Then for any $\delta >0$,  with probability at least $1-2 \delta - 2/n^{10}$, 
\begin{align*}
&(\beta_{\MWLE}-\beta^{\star})^{T}H_w(\beta_{\MWLE}-\beta^{\star}) \\
&\lesssim \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*}
\end{lemma}


The proofs for Lemma \ref{claim1_mis} and \ref{claim2_mis} are delayed to the end of this subsection. With these two lemmas, we can now state the proof for Theorem \ref{thm:mis_upper} and Corollary \ref{cor:mis_upper}.
\begin{proof}[Proof of Theorem \ref{thm:mis_upper}]
By Assumption \ref{assm2}, we can do Taylor expansion w.r.t. $\beta$ as the following:
\begin{align*}
R_{M}(\beta_{\MWLE})&=  
\bbE_{(x,y) \sim \bbP_{T}(x,y)}\left[\ell(x,y,\beta_{\MWLE})-\ell(x,y,\beta^{\star})\right] \notag \\ &\leq  \bbE_{(x,y) \sim \bbP_{T}(x,y)} [\nabla \ell(x,y,\beta^{\star})]^{T}(\beta_{\MWLE}-\beta^{\star}) \notag \\ 
&+ \frac{1}{2}(\beta_{\MWLE}-\beta^{\star})^{T}H_w(\beta_{\MWLE}-\beta^{\star}) +\frac{WB_{3}}{6}\|\beta_{\MWLE}-\beta^{\star}\|_{2}^{3}. 
\end{align*}
 Using Lemma \ref{claim1_mis} and \ref{claim2_mis}, we know that,  with probability at least $1-2 \delta - 2/n^{10}$, 
\begin{align*}
&(\beta_{\MWLE}-\beta^{\star})^{T}H_w(\beta_{\MWLE}-\beta^{\star}) \\
&\lesssim \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*} and
\begin{align*}
   \|\beta_{\MWLE}-\beta^{\star}\|_{2} \leq \sqrt{\frac{ \Tr(G_w H_w^{-2})\log (n^{10}d)}{n}}.
\end{align*}
Also notice that, $\bbE_{(x,y) \sim \bbP_{T}(x,y)} [\nabla \ell(x,y,\beta^{\star})]=0$. Therefore we have with probability at least $1-2\delta -2/n^{10}$,
\begin{align*} 
R_{M}(\beta_{\MWLE})  &\lesssim \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*}
\end{proof}








\subsubsection{Proofs for Lemma \ref{claim1_mis} and \ref{claim2_mis}}
In the following, we prove Lemma \ref{claim1_mis} and \ref{claim2_mis}. 
\paragraph{Concentrations for gradient and Hessian}
In Lemma \ref{lem:bernstein}, for any matrix $A\in \bbR^{d \times d}$, if we choose $u_{i}:=A(\nabla w(x_i) \ell (x_{i},y_{i}, \beta^{\star}) - \bbE_{\bbP_{S}}[\nabla w(x) \ell (x,y, \beta^{\star})])$, then $u_{1}, \cdots, u_{n}$ satisfies the conditions in Lemma \ref{lem:bernstein} with $v=n\Tr (A^{T}A G_w)$, $b=\|A\|_{2}WB_{1}$. Let $g:= \nabla \ell_{n}(\beta^{\star}) - \nabla \bbE_{\bbP_S} \ell_{n}(\beta^{\star})$, then we have with probability at least $1-\delta$, 
\begin{align*}
    \|Ag\|_{2} \leq \sqrt{\frac{\Tr(A^{T}A G_w)}{n}}+  \sqrt{\frac{8\Tr(A^{T}A G_w) \log \frac{1}{\delta}}{n}}+ \frac{4\|A\|_{2} W B_{1}\log \frac{1}{\delta}}{3n},
\end{align*}
Choose $A= H_w^{-1}$ and $A= H_w^{-\frac{1}{2}}$relatively, we have
\begin{align} \label{ineq:pf:concentration1_mis}
    \|H_w^{-1}g\|_{2} \lesssim \sqrt{\frac{\Tr(G_w H_w^{-2})}{n}}+  \sqrt{\frac{\Tr(G_w H_w^{-2}) \log \frac{1}{\delta}}{n}}+ \frac{\|H_w^{-1}\|_{2}W B_{1}\log \frac{1}{\delta}}{n}
\end{align}
and 
\begin{align} \label{ineq:pf:concentration2_mis}
    \|H_w^{-\frac{1}{2}}g\|_{2} \lesssim \sqrt{\frac{\Tr(G_w H_w^{-1})}{n}}+  \sqrt{\frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n}}+ \frac{\|H_w^{-\frac12}\|_{2}W B_{1}\log \frac{1}{\delta}}{n}
\end{align}
with probability at least $1-\delta$ relatively. For Hessian term we also have corresponding concentration. By matrix Hoeffding, since $\|\nabla^{2} w(x) \ell (x,y, \beta^{\star})\| \leq W B_{2}$, we have: for any $t>0$, $\|\nabla^{2} \ell_{n}(\beta^{\star}) - \nabla^{2} \bbE_{\bbP_S} \ell_{n}(\beta^{\star})\|_{2} \leq t$ with probability at least $1-d e^{-nt^{2}/8W^{2}B_{2}^{2}}$. Note that by definition, $\nabla^{2}\bbE_{\bbP_S} \ell_{n}(\beta^{\star}) = H_w,$ therefore with probability at least $1-\delta$, 
\begin{align} \label{ineq:pf:concentration3_mis}
H_w - \sqrt{\frac{8W^{2}B_{2}^{2}\log \frac{d}{\delta}}{n}} I_{d}   \preceq \nabla^{2} \ell_{n}(\beta^{\star}) \preceq H_w + \sqrt{\frac{8W^{2}B_{2}^{2}\log \frac{d}{\delta}}{n}} I_{d}
\end{align}

With (\ref{ineq:pf:concentration1_mis}), (\ref{ineq:pf:concentration2_mis}) and (\ref{ineq:pf:concentration3_mis}), we are now able to prove Lemma \ref{claim1_mis} and \ref{claim2_mis}. 

\begin{proof}[Proof of Lemma \ref{claim1_mis}]
Let $A_{1}:= \{\text{event s.t. } (\ref{ineq:pf:concentration1_mis}) \text{ holds}\}$,   $A_{2}:= \{\text{event s.t. } (\ref{ineq:pf:concentration2_mis}) \text{ holds}\}$,  $A_{3}:= \{\text{event s.t. } (\ref{ineq:pf:concentration3_mis}) \text{ holds}\}$.  Then we know that $\bbP(A_{i}) \geq 1-\delta$ for $i=1,2,3$. Therefore $\bbP(A_{1} \cap A_{2} \cap A_{3}) \geq 1-3\delta$. Under the event $A_{1} \cap A_{2} \cap A_{3}$, we can do the following Taylor expansion:
\begin{align} \label{ineq:pf:taylor1_mis}
\ell_{n}(\beta) - \ell_{n}(\beta^{\star}) &\leq (\beta - \beta^{\star})^{T} \nabla \ell_{n} (\beta^{\star}) +  \frac{1}{2} (\beta - \beta^{\star})^{T} \nabla^{2} \ell_{n} (\beta^{\star}) (\beta - \beta^{\star}) + \frac{W B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3} \notag \\
& \stackrel{\nabla \bbE_{\bbP_S} \ell_n(\beta^{\star})=0}{=} (\beta - \beta^{\star})^{T} g  +  \frac{1}{2} (\beta - \beta^{\star})^{T} \nabla^{2} \ell_{n} (\beta^{\star}) (\beta - \beta^{\star}) + \frac{W B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3} \notag \\
& \stackrel{\text{by (\ref{ineq:pf:concentration3_mis})}}{\leq} (\beta - \beta^{\star})^{T} g + \frac{1}{2} (\beta - \beta^{\star})^{T} H_w (\beta - \beta^{\star}) + \sqrt{\frac{8W^2 B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\beta-\beta^{\star}\|_{2}^{2} + \frac{W B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3}  \notag \\
& \stackrel{\Delta_{\beta}:=\beta-\beta^{\star}}{=} \Delta_{\beta}^{T}g + \frac{1}{2}\Delta_{\beta}^{T} H_w \Delta_{\beta} + \sqrt{\frac{8W^2 B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} + \frac{W B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3} \notag \\
&= \frac{1}{2}(\Delta_{\beta}-z)^{T} H_w (\Delta_{\beta}-z) - \frac{1}{2}z^{T}H_wz + \sqrt{\frac{8W^{2} B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} + \frac{W B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3}
\end{align} 
where $z:=-H_w^{-1}g$. Similarly
\begin{align} \label{ineq:pf:taylor2_mis}
\ell_{n}(\beta) - \ell_{n}(\beta^{\star}) \geq \frac{1}{2}(\Delta_{\beta}-z)^{T} H_w (\Delta_{\beta}-z) - \frac{1}{2}z^{T}H_w z - \sqrt{\frac{8W^2 B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} - \frac{W B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3}.
\end{align}
Notice that $\Delta_{\beta^{\star}+z} = z$, by (\ref{ineq:pf:concentration1_mis}) and (\ref{ineq:pf:taylor1_mis}), we have
\begin{align} \label{ineq:pf:taylor3_mis}
\ell_{n}(\beta^{\star}+z)- \ell_{n}(\beta^{\star}) \leq - \frac{1}{2}z^{T} H_w z+ \cO(W \tilde{B}\Tr(G_w H_w^{-2})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + (W\tilde{B})^{3}\|H_w^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + (W\tilde{B})^{4}\|H_w^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}),
\end{align}
where $\tilde{B}:=\max \{B_1,B_2,B_3\}$. For any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log\frac{d}{\delta}}{n}})$, by (\ref{ineq:pf:taylor2_mis}), we have
\begin{align} \label{ineq:pf:taylor4_mis}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}) \geq \frac{1}{2}(\Delta_{\beta}-z)^{T} H_w (\Delta_{\beta}-z) - \frac{1}{2}z^{T}H_w z - \cO(W\tilde{B}\Tr(G_w H_w^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5}).
\end{align}
(\ref{ineq:pf:taylor4_mis}) - (\ref{ineq:pf:taylor3_mis}) gives
\begin{align} \label{ineq:pf:taylor5_mis}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z)  &\geq \frac{1}{2}(\Delta_{\beta}-z)^{T} H_w (\Delta_{\beta}-z) \notag \\
&- \cO(W \tilde{B}\Tr(G_w H_w^{-2})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + (W\tilde{B})^{3}\|H_w^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + (W\tilde{B})^{4}\|H_w^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}).
\end{align}
Consider the ellipsoid 
\begin{align*}
\cD:=\{ &\beta \in \bbR^{d} | \frac{1}{2}(\Delta_{\beta}-z)^{T} H_w (\Delta_{\beta}-z) \notag \\
&\leq \cO(W \tilde{B}\Tr(G_w H_w^{-2})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + (W\tilde{B})^{3}\|H_w^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + (W\tilde{B})^{4}\|H_w^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}) \}    
\end{align*}
Then by (\ref{ineq:pf:taylor5_mis}), For any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log\frac{d}{\delta}}{n}}) \cap \cD^{C}$, 
\begin{align} \label{ineq:pf:ellipsoid_mis}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z) > 0.    
\end{align}
% In the following, we will show that $D \subset  \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log(n^{10}d)}{n}})$ with probability at least $1-\frac{1}{n^{10}}$. Notice that we do the above mentioned Taylor expansion under the event $A_{1} \cap A_{2} \cap A_{3}$ which has probability at least $1-3\delta$, if we take $\delta=\frac{1}{n^{10}}$, then we know that 
Notice that by the definition of $\cD$, using $\lambda_{\min}^{-1}(H_w)= \|H_w^{-1}\|_{2}$, we have for any $\beta \in \cD$,
\begin{align*}
\|\Delta_{\beta}-z\|_{2}^{2} \leq \cO(\|H_w^{-1}\|_{2}(W \tilde{B}\Tr(G_w H_w^{-2})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + (W\tilde{B})^{3}\|H_w^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + (W\tilde{B})^{4}\|H_w^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3})).
\end{align*}
Thus for any $\beta \in \cD$, 
\begin{align*}
\|\Delta_{\beta}\|_{2}^{2} &\leq 2(\|\Delta_{\beta}-z\|_{2}^{2}+\|z\|_{2}^{2})    \\
& \stackrel{\text{by} (\ref{ineq:pf:concentration1_mis})}{\leq} \cO(W\tilde{B}\Tr(G_w H_w^{-2})^{1.5}\|H_w^{-1}\|_{2}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + (W\tilde{B})^{3}\|H_w^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + (W\tilde{B})^{4}\|H_w^{-1}\|_{2}^{4}(\frac{\log\frac{d}{\delta}}{n})^{3} \\
&\quad + \frac{\Tr(G_w H_w^{-2})\log \frac{d}{\delta}}{n} + (W\tilde{B})^{2}\|H_w^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2})
\end{align*}
We set $\delta= \frac{1}{n^{10}}$, then we have
\begin{align*}
\|\Delta_{\beta}\|_{2}^{2} \leq \cO(\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n})
\end{align*}
when $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{W\tilde{B}\|H_w^{-1}\|_{2}\sqrt{\Tr(G_w H_w^{-2})}}$, i.e., $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}})$.
In other words, we show that $\cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}})$. Therefore, by (\ref{ineq:pf:ellipsoid_mis}), we know that for any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}}) \cap \cD^{C}$, 
\begin{align*} 
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z) > 0,
\end{align*}
which implies there is a local minimum of $\ell_{n}(\beta)$ in $\cD$. By Assumption \ref{assm3}, we know that the global minimum of $\ell_{n}(\beta)$ is in $\cD$, i.e., 
\begin{align*}
    \beta_{\MWLE} \in \cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}})
\end{align*}
with probability at least $1-\frac{2}{n^{10}}$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{claim2_mis}]
Let $A_{1}:= \{\text{event s.t. } (\ref{ineq:pf:concentration1_mis}) \text{ holds}\}$,   $A_{2}:= \{\text{event s.t. } (\ref{ineq:pf:concentration2_mis}) \text{ holds}\}$,  $A_{3}:= \{\text{event s.t. } (\ref{ineq:pf:concentration3_mis}) \text{ holds}\}$, $A_{4}:= \{ \beta_{\MWLE} \in \cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(G_w H_w^{-2})\log (n^{10}d)}{n}}) \}$. Then by Lemma \ref{claim1_mis}, $\bbP(A_4) \geq 1-2/n^{10}$. Therefore $\bbP(A_1 \cap A_2 \cap A_3 \cap A_4) \geq 1-2\delta-2/n^{10}$. Under $A_1 \cap A_2 \cap A_3 \cap A_4$, $\beta_{\MWLE} \in \cD$, i.e., 
\begin{align*}
\frac{1}{2}(\Delta_{\beta_{\MWLE}}-z)^{T}H_w(\Delta_{\beta_{\MWLE}}-z) \leq \cO(W\tilde{B} \Tr(G_w H_w^{-2})^{1.5}(\frac{\log(n^{10}d)}{n})^{1.5}).
\end{align*}
In other words,
\begin{align} \label{ineq:pf:claim2_mis}
\|H_w^{\frac{1}{2}}(\Delta_{\beta_{\MWLE}}-z)\|_{2}^{2} \leq \cO(W\tilde{B} \Tr(G_w H_w^{-2})^{1.5}(\frac{\log(n^{10}d)}{n})^{1.5}).
\end{align}
Thus we have
\begin{align}
\|H_w^{\frac{1}{2}}(\beta_{\MWLE}-\beta^{\star})\|_{2}^{2} & = \|H_w^{\frac{1}{2}}\Delta_{\beta_{\MWLE}}\|_{2}^{2} \notag \\
& = \|H_w^{\frac{1}{2}}(\Delta_{\beta_{\MWLE}}-z) +H_w^{\frac{1}{2}}z \|_{2}^{2} \notag \\
& \leq 2\|H_w^{\frac{1}{2}}(\Delta_{\beta_{\MWLE}}-z)\|_{2}^{2} + 2\|H_w^{\frac{1}{2}}z \|_{2}^{2} \notag \\
& = 2\|H_w^{\frac{1}{2}}
(\Delta_{\beta_{\MWLE}}-z))\|_{2}^{2} + 2\|H_w^{-\frac{1}{2}}g \|_{2}^{2} \notag \\
& \stackrel{\text{by} (\ref{ineq:pf:claim2_mis}) \text{and} (\ref{ineq:pf:concentration2_mis})}{\lesssim} \frac{\Tr(G_w H_w^{-1}) \log \frac{1}{\delta}}{n} + \notag \\
&\cO ( W \tilde{B} \Tr(G_w H_w^{-2})^{1.5} (\frac{\log (n^{10}d)}{n})^{1.5} + \|H_w^{-1}\|_2 W^2 \tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align}
with probability at least $1-2\delta - 2/n^{10}$.
\end{proof}


==> pf_v1_well_upper_bound.tex <==
\subsection{Proofs for Theorem \ref{thm:well_upper}}
For notation simplicity, through out the proofs for Theorem \ref{thm:well_upper}, let $\cI_T:= \cI_T(\beta^{\star})$, $  \cI_S:= \cI_S(\beta^{\star})$, $B_1:=B_1(\beta^{\star})$, $B_2:=B_2(\beta^{\star})$, $\tilde{B}:=\tilde{B}(\beta^{\star})$.
Without loss of generality, we assume  $\tilde{B}$, $\|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|_2 $, $\Tr(\cI^{-1}_S)$, $\|\cI^{-1}_S\|_2 \geq 1$.
We first state two main lemmas. Informally speaking, Lemma \ref{claim1} shows that $\beta_{\MLE}$ falls in a ball around $\beta^{\star}$ with radius $\sqrt{\frac{\log n}{n}}$. With Lemma \ref{claim1}, Lemma \ref{claim2} gives a high probability bound for $\beta_{\MLE}- \beta^{\star}$. 

\begin{lemma}\label{claim1}
Suppose $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{\tilde{B}(\beta^{\star})\|\cI^{-1}_S(\beta^{\star})\|_{2}\sqrt{\Tr(\cI^{-1}_S(\beta^{\star}))}}$. Under Assumptions \ref{assm1}, \ref{assm2} and \ref{assm3}, we have with probability at least $1-2/n^{10}$,  $\beta_{\MLE}\in\bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_S^{-1})\log (n^{10}d)}{n}})$, where $\tilde{B}:= \max \{B_1,B_2,B_3\}$.
\end{lemma}


\begin{lemma}\label{claim2}
Under same conditions as in Lemma \ref{claim1}. Then for any $\delta >0$,  with probability at least $1-2 \delta - 2/n^{10}$, 
\begin{align*}
&(\beta_{\MLE}-\beta^{\star})^{T}\cI_{T}(\beta_{\MLE}-\beta^{\star}) \\
&\lesssim \frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \cO (  \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*}
\end{lemma}
The proofs for Lemma \ref{claim1} and \ref{claim2} are delayed to the end of this subsection. With these two lemmas, we can now state the proof for Theorem \ref{thm:well_upper} and Corollary \ref{cor:well_upper}.
\begin{proof}[Proof of Theorem \ref{thm:well_upper}]
By Assumption \ref{assm2}, we can do Taylor expansion w.r.t. $\beta$ as the following:
\begin{align*}
R_{\beta^{\star}}(\beta_{\MLE})&=  
\bbE_{\substack{x\sim\bbP_T(X)\\y|x\sim f(y|x;\beta^{\star})}}\left[\ell(x,y,\beta_{\MLE})-\ell(x,y,\beta^{\star})\right] \notag \\ &\leq  \bbE_{\substack{x\sim\bbP_T(X)\\y|x\sim f(y|x;\beta^{\star})}} [\nabla \ell(x,y,\beta^{\star})]^{T}(\beta_{\MLE}-\beta^{\star}) \notag \\ 
&+ \frac{1}{2}(\beta_{\MLE}-\beta^{\star})^{T}\cI_{T}(\beta_{\MLE}-\beta^{\star}) +\frac{B_{3}}{6}\|\beta_{\MLE}-\beta^{\star}\|_{2}^{3}. 
\end{align*}
 Using Lemma \ref{claim1} and \ref{claim2}, we know that,  with probability at least $1-2 \delta - 2/n^{10}$, 
\begin{align*}
&(\beta_{\MLE}-\beta^{\star})^{T}\cI_{T}(\beta_{\MLE}-\beta^{\star}) \\
&\lesssim \frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \cO (  \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})
\end{align*} and
\begin{align*}
   \|\beta_{\MLE}-\beta^{\star}\|_{2} \leq \sqrt{\frac{ \Tr(\cI_S^{-1})\log (n^{10}d)}{n}}.
\end{align*}
Also notice that, $\bbE_{\substack{x\sim\bbP_T(X)\\y|x\sim f(y|x;\beta^{\star})}} [\nabla \ell(x,y,\beta^{\star})]=0$. Therefore we have with probability at least $1-2\delta -2/n^{10}$,
\begin{align*} 
R_{\beta^{\star}}(\beta_{\MLE})  &\lesssim \frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \cO (  \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2}).
\end{align*}
\end{proof}




\subsubsection{Proofs for Lemma \ref{claim1} and \ref{claim2}}
In the following, we prove Lemma \ref{claim1} and \ref{claim2}. 
\paragraph{Concentrations for gradient and Hessian}
A crucial part for the proof is the concentration for several quantities. The following lemma is the Bernstein inequality for random vectors (see Proposition 1.2 in \cite{10.1214/ECP.v17-2079}). 
\begin{lemma} \label{lem:bernstein}
Let $u_{1},\cdots,u_{n}$ be a martingale difference vector sequence (i.e., $\bbE[u_{i}|u_{1},\cdots,u_{i-1}]=0$ for all $i=1, \cdots, n$) such that 
\begin{align*}
    \sum_{i=1}^{n} \bbE[\|u_{i}\|^{2}_{2}|u_{1},\cdots,u_{i-1}] \leq v \quad \text{and } \quad \|u_{i}\|_{2} \leq b
\end{align*}
for all $i=1, \cdots, n$, almost surely. Then for all $t>0$, 
\begin{align*}
    \bbP \left( \|\sum_{i=1}^{n}u_{i}\|_{2} > \sqrt{v} +\sqrt{8vt} +\frac{4bt}{3} \right) \leq e^{-t}.
\end{align*}
\end{lemma}
For any matrix $A\in \bbR^{d \times d}$, if we choose $u_{i}:=A(\nabla \ell (x_{i},y_{i}, \beta^{\star}) - \bbE_{\bbP_{S}}[\nabla \ell (x,y, \beta^{\star})])$, then $u_{1}, \cdots, u_{n}$ satisfies the conditions in Lemma \ref{lem:bernstein} with $v=n\Tr (A^{T}A\cI_{S})$, $b=\|A\|_{2}B_{1}$. Let $g:= \nabla \ell_{n}(\beta^{\star}) - \nabla \ell(\beta^{\star})$, then we have with probability at least $1-\delta$, 
\begin{align*}
    \|Ag\|_{2} \leq \sqrt{\frac{\Tr(A^{T}A\cI_{S})}{n}}+  \sqrt{\frac{8\Tr(A^{T}A\cI_{S}) \log \frac{1}{\delta}}{n}}+ \frac{4\|A\|_{2}B_{1}\log \frac{1}{\delta}}{3n},
\end{align*}
Choose $A= \cI_{S}^{-1}$ and $\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}$ relatively, we have
\begin{align} \label{ineq:pf:concentration1}
    \|\cI_{S}^{-1}g\|_{2} \lesssim \sqrt{\frac{\Tr(\cI_{S}^{-1})}{n}}+  \sqrt{\frac{\Tr(\cI_{S}^{-1}) \log \frac{1}{\delta}}{n}}+ \frac{\|\cI_{S}^{-1}\|_{2}B_{1}\log \frac{1}{\delta}}{n}
\end{align}
and 
\begin{align} \label{ineq:pf:concentration2}
    \|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}g\|_{2} \lesssim \sqrt{\frac{\Tr(\cI_{S}^{-1}\cI_{T})}{n}}+  \sqrt{\frac{\Tr(\cI_{S}^{-1}\cI_{T}) \log \frac{1}{\delta}}{n}}+ \frac{\|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}\|_{2}B_{1}\log \frac{1}{\delta}}{n}
\end{align}
with probability at least $1-\delta$ relatively. For Hessian term we also have corresponding concentration. By matrix Hoeffding, since $\|\nabla^{2} \ell (x,y, \beta^{\star})\| \leq B_{2}$, we have: for any $t>0$, $\|\nabla^{2} \ell_{n}(\beta^{\star}) - \nabla^{2} \ell(\beta^{\star})\|_{2} \leq t$ with probability at least $1-d e^{-nt^{2}/8B_{2}^{2}}$, i.e., with probability at least $1-\delta$, 
\begin{align} \label{ineq:pf:concentration3}
\nabla^{2} \ell(\beta^{\star}) - \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} I_{d}   \preceq \nabla^{2} \ell_{n}(\beta^{\star}) \preceq \nabla^{2} \ell(\beta^{\star}) + \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} I_{d}
\end{align}

With (\ref{ineq:pf:concentration1}), (\ref{ineq:pf:concentration2}) and (\ref{ineq:pf:concentration3}), we are now able to prove Lemma \ref{claim1} and \ref{claim2}. 

\begin{proof}[Proof of Lemma \ref{claim1}]
Let $A_{1}:= \{\text{event s.t. } (\ref{ineq:pf:concentration1}) \text{ holds}\}$,   $A_{2}:= \{\text{event s.t. } (\ref{ineq:pf:concentration2}) \text{ holds}\}$,  $A_{3}:= \{\text{event s.t. } (\ref{ineq:pf:concentration3}) \text{ holds}\}$.  Then we know that $\bbP(A_{i}) \geq 1-\delta$ for $i=1,2,3$. Therefore $\bbP(A_{1} \cap A_{2} \cap A_{3}) \geq 1-3\delta$. Under the event $A_{1} \cap A_{2} \cap A_{3}$, we can do the following Taylor expansion:
\begin{align} \label{ineq:pf:taylor1}
\ell_{n}(\beta) - \ell_{n}(\beta^{\star}) &\leq (\beta - \beta^{\star})^{T} \nabla \ell_{n} (\beta^{\star}) +  \frac{1}{2} (\beta - \beta^{\star})^{T} \nabla^{2} \ell_{n} (\beta^{\star}) (\beta - \beta^{\star}) + \frac{B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3} \notag \\
& \stackrel{\nabla \ell(\beta^{\star})=0}{=} (\beta - \beta^{\star})^{T} g  +  \frac{1}{2} (\beta - \beta^{\star})^{T} \nabla^{2} \ell_{n} (\beta^{\star}) (\beta - \beta^{\star}) + \frac{B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3} \notag \\
& \stackrel{\text{by (\ref{ineq:pf:concentration3})}}{\leq} (\beta - \beta^{\star})^{T} g + \frac{1}{2} (\beta - \beta^{\star})^{T} \cI_{S} (\beta - \beta^{\star}) + \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\beta-\beta^{\star}\|_{2}^{2} + \frac{B_{3}}{6} \|\beta-\beta^{\star}\|_{2}^{3}  \notag \\
& \stackrel{\Delta_{\beta}:=\beta-\beta^{\star}}{=} \Delta_{\beta}^{T}g + \frac{1}{2}\Delta_{\beta}^{T} \cI_{S} \Delta_{\beta} + \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} + \frac{B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3} \notag \\
&= \frac{1}{2}(\Delta_{\beta}-z)^{T} \cI_{S} (\Delta_{\beta}-z) - \frac{1}{2}z^{T}\cI_{S}z + \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} + \frac{B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3}
\end{align} 
where $z:=-\cI_{S}^{-1}g$. Similarly
\begin{align} \label{ineq:pf:taylor2}
\ell_{n}(\beta) - \ell_{n}(\beta^{\star}) \geq \frac{1}{2}(\Delta_{\beta}-z)^{T} \cI_{S} (\Delta_{\beta}-z) - \frac{1}{2}z^{T}\cI_{S}z - \sqrt{\frac{8B_{2}^{2}\log \frac{d}{\delta}}{n}} \|\Delta_{\beta}\|_{2}^{2} - \frac{B_{3}}{6} \|\Delta_{\beta}\|_{2}^{3}.
\end{align}
Notice that $\Delta_{\beta^{\star}+z} = z$, by (\ref{ineq:pf:concentration1}) and (\ref{ineq:pf:taylor1}), we have
\begin{align} \label{ineq:pf:taylor3}
\ell_{n}(\beta^{\star}+z)- \ell_{n}(\beta^{\star}) \leq - \frac{1}{2}z^{T}\cI_{S}z+ \cO(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + \tilde{B}^{3}\|\cI_{S}^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + \tilde{B}^{4}\|\cI_{S}^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}),
\end{align}
where $\tilde{B}:=\max \{B_1,B_2,B_3\}$. For any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log\frac{d}{\delta}}{n}})$, by (\ref{ineq:pf:taylor2}), we have
\begin{align} \label{ineq:pf:taylor4}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}) \geq \frac{1}{2}(\Delta_{\beta}-z)^{T} \cI_{S} (\Delta_{\beta}-z) - \frac{1}{2}z^{T}\cI_{S}z - \cO(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5}).
\end{align}
(\ref{ineq:pf:taylor4}) - (\ref{ineq:pf:taylor3}) gives
\begin{align} \label{ineq:pf:taylor5}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z)  &\geq \frac{1}{2}(\Delta_{\beta}-z)^{T} \cI_{S} (\Delta_{\beta}-z) \notag \\
&- \cO(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + \tilde{B}^{3}\|\cI_{S}^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + \tilde{B}^{4}\|\cI_{S}^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}).
\end{align}
Consider the ellipsoid 
\begin{align*}
\cD:=\{ &\beta \in \bbR^{d} | \frac{1}{2}(\Delta_{\beta}-z)^{T} \cI_{S} (\Delta_{\beta}-z) \notag \\
&\leq \cO(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + \tilde{B}^{3}\|\cI_{S}^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + \tilde{B}^{4}\|\cI_{S}^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3}) \}    
\end{align*}
Then by (\ref{ineq:pf:taylor5}), for any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log\frac{d}{\delta}}{n}}) \cap \cD^{C}$, 
\begin{align} \label{ineq:pf:ellipsoid}
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z) > 0.    
\end{align}
% In the following, we will show that $D \subset  \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log(n^{10}d)}{n}})$ with probability at least $1-\frac{1}{n^{10}}$. Notice that we do the above mentioned Taylor expansion under the event $A_{1} \cap A_{2} \cap A_{3}$ which has probability at least $1-3\delta$, if we take $\delta=\frac{1}{n^{10}}$, then we know that 
Notice that by the definition of $\cD$, using $\lambda_{\min}^{-1}(\cI_{S})= \|\cI_{S}^{-1}\|_{2}$, we have for any $\beta \in \cD$,
\begin{align*}
\|\Delta_{\beta}-z\|_{2}^{2} \leq \cO(\|\cI_{S}^{-1}\|_{2}(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + \tilde{B}^{3}\|\cI_{S}^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + \tilde{B}^{4}\|\cI_{S}^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{3})).
\end{align*}
Thus for any $\beta \in \cD$, 
\begin{align*}
\|\Delta_{\beta}\|_{2}^{2} &\leq 2(\|\Delta_{\beta}-z\|_{2}^{2}+\|z\|_{2}^{2})    \\
& \stackrel{\text{by} (\ref{ineq:pf:concentration1})}{\leq} \cO(\tilde{B}\Tr(\cI_{S}^{-1})^{1.5}\|\cI_{S}^{-1}\|_{2}(\frac{\log\frac{d}{\delta}}{n})^{1.5} + \tilde{B}^{3}\|\cI_{S}^{-1}\|_{2}^{3}(\frac{\log\frac{d}{\delta}}{n})^{2.5} + \tilde{B}^{4}\|\cI_{S}^{-1}\|_{2}^{4}(\frac{\log\frac{d}{\delta}}{n})^{3} \\
&\quad + \frac{\Tr(\cI_{S}^{-1})\log \frac{d}{\delta}}{n} + \tilde{B}^{2}\|\cI_{S}^{-1}\|_{2}^{2}(\frac{\log\frac{d}{\delta}}{n})^{2})
\end{align*}
We set $\delta= \frac{1}{n^{-10}}$, then we have
\begin{align*}
\|\Delta_{\beta}\|_{2}^{2} \leq \cO(\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n})
\end{align*}
when $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{\tilde{B}\|\cI_{S}^{-1}\|_{2}\sqrt{\Tr(\cI_{S}^{-1})}}$, i.e., $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n}})$.
In other words, we show that $\cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n}})$. Therefore, by (\ref{ineq:pf:ellipsoid}), we know that for any $\beta \in \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n}}) \cap \cD^{C}$, 
\begin{align*} 
\ell_{n}(\beta)-\ell_{n}(\beta^{\star}+z) > 0,
\end{align*}
which implies there is a local minimum of $\ell_{n}(\beta)$ in $\cD$. By Assumption \ref{assm3}, we know that the global minimum of $\ell_{n}(\beta)$ is in $\cD$, i.e., 
\begin{align*}
    \beta_{\MLE} \in \cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n}})
\end{align*}
with probability at least $1-\frac{2}{n^{10}}$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{claim2}]
Let $A_{1}:= \{\text{event s.t. } (\ref{ineq:pf:concentration1}) \text{ holds}\}$,   $A_{2}:= \{\text{event s.t. } (\ref{ineq:pf:concentration2}) \text{ holds}\}$,  $A_{3}:= \{\text{event s.t. } (\ref{ineq:pf:concentration3}) \text{ holds}\}$, $A_{4}:= \{ \beta_{\MLE} \in \cD \subset \bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_{S}^{-1})\log (n^{10}d)}{n}}) \}$. Then by Lemma \ref{claim1}, $\bbP(A_4) \geq 1-2/n^{10}$. Therefore $\bbP(A_1 \cap A_2 \cap A_3 \cap A_4) \geq 1-2\delta-2/n^{10}$. Under $A_1 \cap A_2 \cap A_3 \cap A_4$, $\beta_{\MLE} \in \cD$, i.e., 
\begin{align*}
\frac{1}{2}(\Delta_{\beta_{\MLE}}-z)^{T}\cI_{S}(\Delta_{\beta_{\MLE}}-z) \leq \cO(\tilde{B} \Tr(\cI_{S}^{-1})^{1.5}(\frac{\log(n^{10}d)}{n})^{1.5}).
\end{align*}
In other words,
\begin{align} \label{ineq:pf:claim2}
\|\cI_{S}^{\frac{1}{2}}(\Delta_{\beta_{\MLE}}-z)\|_{2}^{2} \leq \cO(\tilde{B} \Tr(\cI_{S}^{-1})^{1.5}(\frac{\log(n^{10}d)}{n})^{1.5}).
\end{align}
Thus we have
\begin{align}
\|\cI_{T}^{\frac{1}{2}}(\beta_{\MLE}-\beta^{\star})\|_{2}^{2} & = \|\cI_{T}^{\frac{1}{2}}\Delta_{\beta_{\MLE}}\|_{2}^{2} \notag \\
& = \|\cI_{T}^{\frac{1}{2}}(\Delta_{\beta_{\MLE}}-z) +\cI_{T}^{\frac{1}{2}}z \|_{2}^{2} \notag \\
& \leq 2\|\cI_{T}^{\frac{1}{2}}(\Delta_{\beta_{\MLE}}-z)\|_{2}^{2} + 2\|\cI_{T}^{\frac{1}{2}}z \|_{2}^{2} \notag \\
& = 2\|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-\frac{1}{2}} (\cI_{S}^{\frac{1}{2}}
(\Delta_{\beta_{\MLE}}-z))\|_{2}^{2} + 2\|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}g \|_{2}^{2} \notag \\
& \leq 2\|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-\frac{1}{2}}\|_{2}^{2}\|(\cI_{S}^{\frac{1}{2}}
(\Delta_{\beta_{\MLE}}-z))\|_{2}^{2} + 2\|\cI_{T}^{\frac{1}{2}}\cI_{S}^{-1}g \|_{2}^{2} \notag \\
& \stackrel{\text{by} (\ref{ineq:pf:claim2}) \text{and} (\ref{ineq:pf:concentration2})}{\lesssim} \frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \notag \\
&\cO (\tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})  
\end{align}
with probability at least $1-2\delta - 2/n^{10}$.
\end{proof}

==> pf_well_expectation_upper.tex <==
\subsection{Expectation upper bound}\label{well:expectation_upper}
If we are given prior knowledge that $\beta^{\star}\in\bbB_{\beta_0}(B)$ for some $\beta_0\in\bbR^{d}$ and $B>0$, then we consider the following constrained MLE:
\begin{align*}
\tilde{\beta}_{\MLE}:=\argmin_{\beta\in\bbB_{\beta_0}(2B)}\frac1n \sum^n_{i=1}\ell(x_i,y_i,\beta).   
\end{align*}


% \begin{corollary}\label{cor:well_upper}
% Suppose $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \min \left\{ \frac{1}{\tilde{B}(\beta^{\star})\|\cI^{-1}_S(\beta^{\star})\|_{2}\sqrt{\Tr(\cI^{-1}_S(\beta^{\star}))}}, \frac{B}{\sqrt{\Tr(\cI^{-1}_S(\beta^{\star}))}} \right\}$. Under Assumptions \ref{assm1}, \ref{assm2} and \ref{assm3}, we have
% \begin{align*}
% \bbE_{\substack{x_i\sim\bbP_S(X)\\y_i|x_i\sim f(y|x;\beta^{\star})}}\left[R_{\beta^{\star}}(\tilde{\beta}_{\MLE})\right] &\leq \frac{c\Tr\left(\cI_T(\beta^{\star})\cI^{-1}_S(\beta^{\star})\right)}{n} \\
% &+ \cO \left(\tilde{B}(\beta^{\star}) \|\cI_T^{\frac{1}{2}}(\beta^{\star})\cI^{-\frac{1}{2}}_S(\beta^{\star})\|_2^{2}   \Tr(\cI^{-1}_S(\beta^{\star}))^{1.5} \left(\frac{\log (n^{10}d)}{n}\right)^{1.5} + \frac{\tilde{B}(\beta^{\star})B^{3}\|\cI_T(\beta^{\star})\|_2 }{n^{10}} \right)
% \end{align*}
% where $\tilde{B}(\beta^{\star}) := \max \{B_1(\beta^{\star}), B_2(\beta^{\star}), B_3\},$
% $c$ is an absolute constant and $\cO(\cdot)$ only omits absolute constants.
% \end{corollary}

\begin{corollary}\label{cor:well_upper}
Suppose Assumptions \ref{assm1}, \ref{assm2} and \ref{assm3} hold. We have
\begin{align*}
\bbE_{\substack{x_i\sim\bbP_S(X)\\y_i|x_i\sim f(y|x;\beta^{\star})}}\left[R_{\beta^{\star}}(\tilde{\beta}_{\MLE})\right] \lesssim\frac{\Tr\left(\cI_T(\beta^{\star})\cI^{-1}_S(\beta^{\star})\right)}{n}
\end{align*}
when
\begin{align*}
n\gtrsim \max\bigg\{
&\tilde{B}(\beta^{\star})^2\|\cI^{-1}_S(\beta^{\star})\|^2_{2}\Tr(\cI^{-1}_S(\beta^{\star}))\log d \tilde{B}(\beta^{\star})\|\cI^{-1}_S(\beta^{\star})\|_{2}\Tr(\cI^{-1}_S(\beta^{\star})),\\
& \frac{\tilde{B}(\beta^{\star})^2 \|\cI_T^{\frac{1}{2}}(\beta^{\star})\cI^{-\frac{1}{2}}_S(\beta^{\star})\|_2^{4}   \Tr(\cI^{-1}_S(\beta^{\star}))^{3}}{\Tr\left(\cI_T(\beta^{\star})\cI^{-1}_S(\beta^{\star})\right)^2}\left(\log d \tilde{B}(\beta^{\star}) \|\cI_T^{\frac{1}{2}}(\beta^{\star})\cI^{-\frac{1}{2}}_S(\beta^{\star})\|_2   \Tr(\cI^{-1}_S(\beta^{\star}))\right)^3
\bigg\}.
\end{align*}
Here $\tilde{B}(\beta^{\star}) := \max \{B_1(\beta^{\star}), B_2(\beta^{\star}), B_3\}$.
\end{corollary}
\jiawei{Need to change!}
\begin{proof}[Proof of Corollary \ref{cor:well_upper}]
In the proof of Theorem \ref{thm:well_upper}, we already have with probability at least $1-2\delta -2/n^{10}$,
\begin{align*} 
R_{\beta^{\star}}(\beta_{\MLE})  &\lesssim \frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \cO (  \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2}).
\end{align*}
Also notice that, under this event, since $\sqrt{\frac{\Tr(\cI_S^{-1})\log (n^{10}d)}{n}} \leq B$, by Lemma \ref{claim1}, $\beta_{\MLE}\in\bbB_{\beta^{\star}}(\sqrt{\frac{\Tr(\cI_S^{-1})\log (n^{10}d)}{n}}) \subset \bbB_{\beta_{0}}(2B)$. Thus $\beta'_{\MLE}=\beta_{\MLE}$. Therefore we have with probability at least $1-2\delta -2/n^{10}$, 
\begin{align}\label{ineq:pf:upper1} 
&R_{\beta^{\star}}(\beta'_{\MLE})  \notag\\
&\lesssim \underbrace{\frac{\Tr(\cI_{T} \cI_{S}^{-1}) \log \frac{1}{\delta}}{n} + \cO (  \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log \frac{1}{\delta}}{n})^{2})}_{=:f(\delta)}.
\end{align}
Taking the expectation, we have
\begin{align} \label{ineq:pf:upper2}
& \bbE_{\substack{x_i\sim\bbP_S(X)\\y_i|x_i\sim f(y|x;\beta^{\star})}}\left[R_{\beta^{\star}}(\beta_{\MLE})\right] \notag \\
& = \int_{0}^{+\infty} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t \notag \\
&= \underbrace{\int_{0}^{f(1)} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t }_{=
:K_1}+ \underbrace{\int_{f(1)}^{f(\frac{1}{n^{10}})} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t }_{=:K_2}+ \underbrace{\int_{f(\frac{1}{n^{10}})}^{+\infty} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t }_{=:K_3}.
\end{align}
We will relatively bound these three terms $K_1, K_2, K_3$.
Note that
\begin{align} \label{ineq:pf:upper3}
K_{1} &=  \int_{0}^{f(1)} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t \notag \\
& \leq \int_{0}^{f(1)} 1 \mathrm{d}t \notag \\
&= f(1) \notag \\
&= \cO \left( \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5}\right),
\end{align}
where the last equality holds because of the definition of $f(\delta)$  (see \eqref{ineq:pf:upper1}).

\begin{align} \label{ineq:pf:upper4}
K_2 &= \int_{f(1)}^{f(\frac{1}{n^{10}})} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t \notag \\
&\stackrel{\text{let } t=f(\delta)}{=} -\int_{\frac{1}{n^{10}}}^{1} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq f(\delta)) f'(\delta) \mathrm{d}\delta \notag \\
& \stackrel{\text{by (\ref{ineq:pf:upper1}})}{\leq} -\int_{\frac{1}{n^{10}}}^{1} (2\delta + \frac{2}{n^{10}}) f'(\delta) \mathrm{d}\delta \notag \\
& = - 2\int_{\frac{1}{n^{10}}}^{1} \delta f'(\delta) \mathrm{d}\delta - \frac{2}{n^{10}} \int_{\frac{1}{n^{10}}}^{1} f'(\delta) \mathrm{d}\delta \notag \\
&= - 2\int_{\frac{1}{n^{10}}}^{1} \delta \frac{c \Tr(\cI_{T} \cI_{S}^{-1})}{n} \delta (-\frac{1}{\delta^{2}}) \mathrm{d}\delta -\frac{1}{n^{2}} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} \int_{\frac{1}{n^{10}}}^{1} \cO \left(\delta^{2}(-\frac{1}{\delta^{2}}) \log \frac{1}{\delta}\right) \mathrm{d}\delta - \frac{2}{n^{10}} (f(1)-f(\frac{1}{n^{10}})) \notag \\
&\leq  \frac{2c \Tr(\cI_{T} \cI_{S}^{-1})}{n} + \frac{1}{n^{2}} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} \int_{0}^{1} \cO(\log \frac{1}{\delta})\mathrm{d}\delta + \frac{2}{n^{10}} f(\frac{1}{n^{10}}) \notag \\
& = \frac{2c \Tr(\cI_{T} \cI_{S}^{-1})}{n} + \cO(\frac{1}{n^{2}} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2})\notag\\
&\quad + \frac{1}{n^{10}}\cO ( \tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5} + \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2} (\frac{\log n}{n})^{2})\notag \\
& \leq \frac{2c \Tr(\cI_{T} \cI_{S}^{-1})}{n} + \cO(\frac{1}{n^{2}} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 \|\cI^{-1}_S\|_2\tilde{B}^{2}),
\end{align}
where the last inequality follows from $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{\tilde{B}(\beta^{\star})\|\cI^{-1}_S(\beta^{\star})\|_{2}\sqrt{\Tr(\cI^{-1}_S(\beta^{\star}))}}$.


Note that $\beta^{\star}, \beta_{\MLE} \in \bbB_{\beta_{0}}(2B)$, we have a trivial bound
\begin{align*}
R_{\beta^{\star}}(\beta_{\MLE}) \leq \frac{1}{2}(\beta_{\MLE}-\beta^{\star})^{T}\cI_{T}(\beta_{\MLE}-\beta^{\star}) +\frac{B_{3}}{6}\|\beta_{\MLE}-\beta^{\star}\|_{2}^{3} \lesssim \|\cI_{T}\|_{2}\tilde{B}B^{3}.
\end{align*}
Thus 
\begin{align} \label{ineq:pf:upper5}
K_3 &= \int_{f(\frac{1}{n^{10}})}^{+\infty} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq t) \mathrm{d}t \notag \\
& = \bbE_{\substack{x_i\sim\bbP_S(X)\\y_i|x_i\sim f(y|x;\beta^{\star})}}\left[(R_{\beta^{\star}}(\beta_{\MLE})- f(\frac{1}{n^{10}})) \bbI_{(R_{\beta^{\star}}(\beta_{\MLE})- f(\frac{1}{n^{10}})\geq 0)}\right] \notag \\
& \leq \|\cI_{T}\|_{2}\tilde{B}B^{3} \bbP(R_{\beta^{\star}}(\beta_{\MLE}) \geq f(\frac{1}{n^{10}})) \notag \\
& \lesssim \frac{1}{n^{10}}\|\cI_{T}\|_{2}\tilde{B}B^{3}
\end{align}
Combine  (\ref{ineq:pf:upper2}), (\ref{ineq:pf:upper3}), (\ref{ineq:pf:upper4}) and (\ref{ineq:pf:upper5}), notice that $\sqrt{\frac{\log (n^{10}d)}{n}} \lesssim \frac{1}{\tilde{B}(\beta^{\star})\|\cI^{-1}_S(\beta^{\star})\|_{2}\sqrt{\Tr(\cI^{-1}_S(\beta^{\star}))}}$, we have 
\begin{align*}
&\bbE_{\substack{x_i\sim\bbP_S(X)\\y_i|x_i\sim f(y|x;\beta^{\star})}}\left[R_{\beta^{\star}}(\beta_{\MLE})\right] \leq \frac{c \Tr(\cI_{T} \cI_{S}^{-1})}{n} + \cO \left(\tilde{B} \Tr(\cI^{-1}_S)^{1.5} \|\cI^{\frac{1}{2}}_T\cI^{-\frac{1}{2}}_S\|^{2}_2 (\frac{\log (n^{10}d)}{n})^{1.5}+ \frac{\|\cI_{T}\|_{2}\tilde{B}B^{3}}{n^{10}}\right),
\end{align*}
where $c$ is an absolute constant and $\cO(\cdot)$ only omits absolute constants.
\end{proof}




==> vector_concentration_v1.tex <==
\subsection{Vector concentrations}
\begin{lemma}\label{lem:concentration_vec}
Suppose $p\in\{1,2,\infty\}$. Let $u_{1},\cdots,u_{n}$ be i.i.d. mean-zero random vectors such that 
\begin{align*}
    \bbE[\|u_{i}\|^{2}_{2}] \leq v \quad \text{and } \quad \bbP(\|u_{i}\|_{2} \geq t) \leq 2e^{-\frac12(\frac{t}{B})^p}
\end{align*}
for all $i=1, \cdots, n$. Then for any $\delta \in [n^{-10},e^{-1}]$, with probability at least $1-\delta$, we have
\begin{align*}
     \left\|\frac{1}{n}\sum_{i=1}^{n}u_{i}\right\|_{2} \leq c  \left(\sqrt{\frac{v\log \frac{1}{\delta}}{n}}+\frac{B(\log n)^{\frac1p}\log \frac{1}{\delta}}{n}\right).
\end{align*}
\end{lemma}


% \subsection{Matrix concentrations}

% \begin{lemma}\label{lem:concentration_matrix}
% Let $A_{1},\cdots,A_{n}$ be i.i.d. symmetric random matrices such that 
% \begin{align*}
%     \bbP(\|A_{i}\|_{2} \geq t) \leq 2e^{-\frac12(\frac{t}{B})^p}\end{align*}
% for all $i=1, \cdots, n$. Then for any $\delta \in (0,e^{-1})$, with probability at least $1-2n^{-10}-\delta$, we have
% \begin{align*}
%      \left\|\frac{1}{n}\sum_{i=1}^{n}A_{i}-\bbE[A_i]\right\|_{2} \lesssim  B(\log n)^{\frac1p}\sqrt{\frac{\log \frac{d}{\delta}}{n}},
% \end{align*}
% i.e.,
% \begin{align*}
%     \bbE[A_i]-B(\log n)^{\frac1p}\sqrt{\frac{\log \frac{d}{\delta}}{n}}\cdot I_d \precsim\frac{1}{n}\sum_{i=1}^{n}A_{i}\precsim \bbE[A_i]+B(\log n)^{\frac1p}\sqrt{\frac{\log \frac{d}{\delta}}{n}}\cdot I_d
% \end{align*}
% \end{lemma}

% \subsection{Proof of Lemma \ref{lem:bernstein}}\label{pf:lem_bernstein}
\begin{proof}[Proof of Lemma \ref{lem:concentration_vec}]
When $p=\infty$, we have $\|u_i\|_2\leq B$. Under this scenario, Lemma \ref{lem:concentration_vec} directly follows from Proposition 2 in \cite{hsu2012tail}.

In the following, we prove Lemma \ref{lem:concentration_vec} for $p=1,2$.


Let $\tilde{u}_i := u_i \bbI_{\{ \|u_i\| \leq B(22\log n)^{1/p}\}} $. 
By the tail property of $\|u_i\|$, we have 
\begin{align*}
\bbP(\exists i \in [n], \, s.t. \, \|u_i\| \geq B(22\log n)^{1/p})     &\leq \sum_{i=1}^{n} \bbP( \|u_i\| \geq B(22\log n)^{1/p}) \\
&\leq n \times 2 e^{-11\log n} \\
& = \frac{2}{n^{10}}.
\end{align*}
Note that
\begin{align*}
\|\bbE [\tilde{u}_i]\| &= \|\bbE[u_i] - \bbE [u_i\bbI_{\{ \|u_i\| > B(22\log n)^{1/p}\}}] \| \\ 
&\stackrel{\bbE[u_i]=0}{=} \|\bbE [u_i\bbI_{\{ \|u_i\| >B(22\log n)^{1/p}\}}] \| \\ 
& \leq \bbE [\|u_i\|\bbI_{\{ \|u_i\| \geq B(22\log n)^{1/p}\}}]  \\
&= \int_{B(22\log n)^{1/p}}^{\infty} \bbP(\|u_i\|\geq t) \mathrm{d} t  + B(22\log n)^{1/p} \bbP(\|u_i\| \geq B(22\log n)^{1/p}) \\
& \leq \int_{B(22\log n)^{1/p}}^{\infty} 2e^{-\frac12 (\frac{t}{B})^{p}} \mathrm{d} t  + \frac{2}{n^{11}}B(22\log n)^{1/p}  
% & \stackrel{\text{let } t=Bs}{=} \int_{\sqrt{22 \log n}}^{\infty} 2Be^{-\frac{s^{2}}{2}} \mathrm{d} s  + \frac{2}{n^{11}}B(22\log n)^{1/p}  \\
% &= cB \bbP(\cN (0,1) \geq \sqrt{22 \log n})  + \frac{2}{n^{11}}B(22\log n)^{1/p} \\
% & \stackrel{\text{by Gaussian tail bound}}{\leq} cB e^{-\frac{22\log n }{2}}+ \frac{2}{n^{11}}B(22\log n)^{1/p} \\
% & \leq CB \frac{\sqrt{\log n}}{n^{11}}.
\end{align*}
When $p=1$, we have
\begin{align*}
 \int_{B(22\log n)^{1/p}}^{\infty} 2e^{-\frac12 (\frac{t}{B})^{p}} \mathrm{d} t =    \int_{22B\log n}^{\infty} 2e^{-\frac{t}{2B}} \mathrm{d} t =\frac{4B}{n^{11}}.
\end{align*}
When $p=2$, we have
\begin{align*}
 \int_{B(22\log n)^{1/p}}^{\infty} 2e^{-\frac12 (\frac{t}{B})^{p}} \mathrm{d} t
 &=    \int_{B(22\log n)^{1/2}}^{\infty} 2e^{-\frac12 (\frac{t}{B})^{2}} \mathrm{d} t\notag\\
 & \stackrel{\text{let } t=Bs}{=} \int_{\sqrt{22 \log n}}^{\infty} 2Be^{-\frac{s^{2}}{2}} \mathrm{d} s \\
&= cB \bbP(\cN (0,1) \geq \sqrt{22 \log n})   \\
& \stackrel{\text{by Gaussian tail bound}}{\leq} cB e^{-\frac{22\log n }{2}} \\
& =  \frac{cB}{n^{11}}.
\end{align*}
Hence for $p=1,2$ and an absoulte constant $c$, we have 
\begin{align*}
\|\bbE [\tilde{u}_i]\| \leq  cB \frac{(\log n)^{1/p}}{n^{11}}.   
\end{align*}
Thus 
\begin{align*}
\|\tilde{u}_i - \bbE \tilde{u}_i\| &\leq \|\tilde{u}_i\|+ \|\bbE \tilde{u}_i\| \\
& \leq B(22\log n)^{1/p}+ cB \frac{(\log n)^{1/p}}{n^{11}} \\
& \leq cB (\log n)^{1/p}.
\end{align*}
Moreover, 
\begin{align*}
\bbE[\|\tilde{u}_i - \bbE \tilde{u}_i\|^{2}] = \bbE[\|\tilde{u}_i\|^{2}] -\| \bbE \tilde{u}_i\|^{2} \leq \bbE[\|\tilde{u}_i\|^{2}] \leq \bbE[\|u_i\|^{2}]\leq v.
\end{align*}
By Proposition 2 in \cite{10.1214/ECP.v17-2079}, 
% we have the following Bernstein inequality:
% \begin{lemma} \label{lem:bernstein2}
% Let $u_{1},\cdots,u_{n}$ be a martingale difference vector sequence (i.e., $\bbE[u_{i}|u_{1},\cdots,u_{i-1}]=0$ for all $i=1, \cdots, n$) such that 
% \begin{align*}
%     \sum_{i=1}^{n} \bbE[\|u_{i}\|^{2}_{2}|u_{1},\cdots,u_{i-1}] \leq v \quad \text{and } \quad \|u_{i}\|_{2} \leq b
% \end{align*}
% for all $i=1, \cdots, n$, almost surely. Then for all $t>0$, 
% \begin{align*}
%     \bbP \left( \|\sum_{i=1}^{n}u_{i}\|_{2} > \sqrt{v} +\sqrt{8vt} +\frac{4bt}{3} \right) \leq e^{-t}.
% \end{align*}
% \end{lemma}
% Apply Lemma \ref{lem:bernstein2} to $\tilde{u}_i - \bbE \tilde{u}_i$ as the random vector sequence, 
we have
\begin{align*}
\bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i - \bbE \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p} \log \frac{1}{\delta}}{3n}) \leq \delta,
\end{align*}
which implies 
\begin{align*}
\bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}}) \leq \delta,
\end{align*}
since $\|\bbE \tilde{u}_i\| \leq  cB \frac{(\log n)^{1/p}}{n^{11}}$. Thus, for any $\delta\geq n^{-10}$, we have
\begin{align*}
& \bbP (\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}})   \\
&= \bbP (\{\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}}\} \cap \{\exists i \in [n], \, s.t. \, \|u_i\| \geq B(22\log n)^{1/p}\}) \\
&+\bbP (\{\|\frac{1}{n} \sum_{i=1}^{n} u_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}}\}\cap \{\forall i \in [n], \,  \, \|u_i\| < B(22\log n)^{1/p}\})  \\
& \leq \bbP(\exists i \in [n], \, s.t. \, \|u_i\| \geq B(22\log n)^{1/p}) + \bbP (\|\frac{1}{n} \sum_{i=1}^{n} \tilde{u}_i \| > \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}})   \\
& \leq \frac{2}{n^{10}} + \delta\\
&\leq 3\delta.
\end{align*}
Notice that for $\delta \leq e^{-1}$, $\log \frac{1}{\delta} \geq 1$. Thus, for any $\delta\in [n^{-10},e^{-1}]$, we have with probability at least $1-3\delta$,
\begin{align*}
\|\frac{1}{n} \sum_{i=1}^{n} {u}_i \| &\leq \sqrt{\frac{v}{n}} + \sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{4cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} + cB \frac{(\log n)^{1/p}}{n^{11}}\\
&\leq 2\sqrt{\frac{8v \log \frac{1}{\delta}}{n}} + \frac{7cB (\log n)^{1/p}\log \frac{1}{\delta}}{3n} \\
&\leq c  \left(\sqrt{\frac{v\log \frac{1}{\delta}}{n}}+\frac{B(\log n)^{\frac1p}\log \frac{1}{\delta}}{n}\right).
\end{align*}
\end{proof}

